SAFE-SIM: Safety-Critical Closed-Loop Traffic Simulation with Diffusion-Controllable Adversaries

Evaluating the performance of autonomous vehicle planning algorithms necessitates simulating long-tail safety-critical traffic scenarios. However, traditional methods for generating such scenarios often fall short in terms of controllability and realism; they also neglect the dynamics of agent interactions. To address these limitations, we introduce SAFE-SIM, a novel diffusion-based controllable closed-loop safety-critical simulation framework. Our approach yields two distinct advantages: 1) generating realistic long-tail safety-critical scenarios that closely reflect real-world conditions, and 2) providing controllable adversarial behavior for more comprehensive and interactive evaluations. We develop a novel approach to simulate safety-critical scenarios through an adversarial term in the denoising process of diffusion models, which allows an adversarial agent to challenge a planner with plausible maneuvers while all agents in the scene exhibit reactive and realistic behaviors. Furthermore, we propose novel guidance objectives and a partial diffusion process that enables users to control key aspects of the scenarios, such as the collision type and aggressiveness of the adversarial agent, while maintaining the realism of the behavior. We validate our framework empirically using the nuScenes and nuPlan datasets across multiple planners, demonstrating improvements in both realism and controllability. These findings affirm that diffusion models provide a robust and versatile foundation for safety-critical, interactive traffic simulation, extending their utility across the broader autonomous driving landscape. Project website: https://safe-sim.github.io/.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> reb_tbl/diff_planner_reb.tex <==
\setlength\tabcolsep{5 pt}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccc} 
\toprule
\textbf{Planner} & \textbf{Ego-Adv Coll} & \textbf{Ego-Other Coll} & \textbf{Adv Offroad} & \textbf{Coll Speed} & \textbf{Ego Accel }     & \textbf{Realism}  \\
                                      & (\%) $\uparrow$        & (\%) $\uparrow$         & (\%) $\downarrow$     & (m/s) $\downarrow$  & (m/s$^2$) $\downarrow$ & $\downarrow$      \\ 
\midrule
BC                                    & 40.3                  & 43.3                    & 20.9                 & 2.65                & \textbf{0.60}           & 0.83              \\
IDM                                   & \textbf{49.3}         & \textbf{58.2}           & 15.0                 & \textbf{-0.37}      & 1.09                    & 0.85              \\
Lane-Graph                            & 35.8                  & 38.8                    & \textbf{13.4}        & 2.34                & 2.51                    & 0.60              \\
BITS              & 17.9                  & 25.4                    & 23.9                 & 3.33                & 1.19                    & \textbf{0.54}     \\
PDM-Closed             &    7.2               &         21.7             &  24.6                 &         0.93       &         2.26              &  0.55  \\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\captionof{table}{\textbf{Safety-Critical Simulation for different Planners.}\vspace{-1.25em}}
\label{tab:reb_diffplan}
\end{table}

\setlength\tabcolsep{6 pt}

==> reb_tbl/diffscene_baseline.tex <==
\setlength\tabcolsep{3 pt}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|cccccc} 
\toprule
\textbf{Dataset} & \textbf{Method} & \textbf{Collision} & \textbf{Other Offroad}    & \textbf{Adv Offroad}      & \textbf{Collision Rel Speed} & \textbf{Realism}  & \textbf{DTW} \\
                             
                               &  & (\%) $\uparrow$                     & (\%) $\downarrow$ & (\%) $\downarrow$ & (m/s) $\downarrow$ & $\downarrow$    &       $\downarrow$             \\ 
\midrule

% \multirow{3}{*}{nuScenes}  & Strive                           & 36.3                                & 2.2               & 11.4              & 6.56               & 0.80                               \\
\multirow{2}{*}{nuScenes} & Ours                             & \textbf{43.2}                                & \textbf{1.8}      & 11.4              & \textbf{-0.12}              & \textbf{0.38}    & \textbf{27.5}                  \\
& DiffScene          & 18.2                                & 11.4              & \textbf{9.0}               & 16.4               & 0.52              & 29.7                  \\
\midrule
\multirow{2}{*}{nuPlan} & Ours & \textbf{80} & \textbf{9.4} & 11.7  & 6.75  & \textbf{0.27} & \textbf{21.3} \\
& DiffScene & 56.7  & 14.0  & \textbf{5.0}   & \textbf{-2.81}  & 0.42 & 43.6\\

% \midrule
%  & Ours & 63.3 & 8.8  & 11.7 & 7.29     & 0.38   &  24.9                         \\
%  & DiffScene & 61.7  & 16.5  & 25.0   & 3.47  & 0.93  & 93.5 \\
\bottomrule
\end{tabular}
}
\vspace{-.75em}
\caption{\textbf{Comparison to another baseline (DiffScene) and implementation on another dataset (nuPlan).} }
\label{tab:reb_nuscene}
\end{table}
\setlength\tabcolsep{6 pt}





% % \setlength\tabcolsep{4 pt}

% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|ccccc} 
% \toprule
% \textbf{Method} & \textbf{Collision} & \textbf{Other Offroad}    & \textbf{Adv Offroad}      & \textbf{Collision Rel Speed} & \textbf{Realism}  \\
                             
%                                  & (\%) $\uparrow$                     & (\%) $\downarrow$ & (\%) $\downarrow$ & (m/s) $\downarrow$ & $\downarrow$                       \\ 
% \midrule
% % Strive                           & 36.3                                & 2.2               & 11.4              & 6.56               & 0.80                               \\
% Ours                             & 43.2                                & \textbf{1.8}      & 11.4              & -0.12              & \textbf{0.38}                      \\
% DiffScene          & 18.2                                & 11.4              & 9.0               & 16.4               & 0.52                               \\
% % DiffScene (open-loop)            & 29.5                                & 11.9              & 9.0               & \textbf{-2.1}      & 0.74                               \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-.75em}
% \caption{\textbf{Safety-Critical Simulation on NuScenes.}  \vspace{-1em}}
% \label{tab:reb_nuscene}
% \end{table}
% \setlength\tabcolsep{6 pt}




==> tbl/abl.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\label{tab:scenario_generation_metrics}
\begin{tabular}{lcccccc} 
\toprule
\textbf{Model}       & \textbf{Collision (\%)} & \textbf{Off-road (\%)} & \textbf{Progress (m)} & \textbf{Wrong Direction(\%)} & \textbf{Realism} \\ 
\midrule
Ours (- $J_{gc}$)    & 30.82  & 0.46  & 48.1 & \textbf{8.72}        & 0.71   \\
Ours (- $J_{route}$)       & \textbf{3.03}   & 3.48& 51.2 & 23.9        & 1.08  \\
Ours (- clean guide) & 5.15   & \textbf{0.32}  & 11.8& 4.65        & \textbf{0.55}     \\
Ours& 4.21   & 1.15  & \textbf{56.8} & 9.37        & 0.96   \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation study on diffusion model guidance functions.} Results show the effectiveness of $J_{gc}$ in reducing collision rates, the role of $J_{route}$ in managing wrong-direction incidents, and the impact of clean guidance on improving the progress of reactive agents.}
\label{tab:abl}
\vspace{-1em}
\end{table}



% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{%
% \label{tab:scenario_generation_metrics}
% \begin{tabular}{lcccccc} 
% \toprule
% \textbf{Model}       & \textbf{Collision (\%)} & \textbf{Off-road (\%)} & \textbf{Progress (m)} & \textbf{Wrong Direction(\%)} & \textbf{Realism} \\ 
% \midrule
% Ours (- $J_{gc}$)    & 30.82  & 0.46  & 48.1 & \textbf{8.72}        & 0.71   \\
% Ours (- $J_{route}$)       & \textbf{3.03}   & 3.48& 51.2 & 23.9        & 1.08  \\
% Ours (- clean guide) & 5.15   & \textbf{0.32}  & 11.8& 4.65        & \textbf{0.55}     \\
% Ours& 4.21   & 1.15  & \textbf{56.8} & 9.37        & 0.96   \\
% \bottomrule
% \end{tabular}
% }
% \caption{\textbf{Ablation study on diffusion model guidance functions.} Results show the effectiveness of $J_{gc}$ in reducing collision rates, the role of $J_{route}$ in managing wrong-direction incidents, and the impact of clean guidance on improving the progress of reactive agents.}
% \label{tab:abl}
% \vspace{-1em}
% \end{table}


==> tbl/adv_sup.tex <==
\setlength\tabcolsep{4 pt}
\begin{table}[t]
% \begin{center}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccc} 
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Ego-Adv Coll} & \textbf{Ego-Other Coll} & \textbf{Other Offroad} & \textbf{Adv Offroad} & \textbf{Coll Speed} & \textbf{Realism}  \\
       & (\%) $\uparrow$       & (\%) $\uparrow$         & (\%) $\downarrow$      & (\%) $\downarrow$    & (m/s) $\downarrow$  & $\downarrow$      \\ 
\midrule
Ours (- $J_{route}$)~ & 47.1     & 50.0       & 25.5      & 28.0    & \textbf{2.19}       & 0.56 \\
Ours~ (- clean guide)            & \textbf{51.2}         & \textbf{51.2}           & \textbf{14.6}          & 17.1    & 2.20   & 0.61 \\
Ours   & 38.2     & 42.7       & 23.2      & \textbf{8.8}         & 2.63   & \textbf{0.48}     \\
\bottomrule
\end{tabular}
}
\captionof{table}{\textbf{Ablation study on diffusion model guidance functions for safety-critical simulation.}We compare the performance of our approach with and without our proposed ``route'' and ``clean'' guidance functions when generating safety-critical traffic simulations. Our guidance lead to enhanced performance in Ego-Adversary collision rate with reduced adversary's off-road rate and improved realism}
\label{tab:supp_adv}
\end{table}

==> tbl/ctg.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc} 
\toprule
 \multirow{2}{*}{\textbf{Method}}   & \textbf{Coll Rate} &\textbf{Off Road } &\textbf{Failure Rate} &\textbf{Wrong Direction} & \textbf{Realism} \\ 
   & (\%) $\downarrow$ & (\%) $\downarrow$ & (\%) $\downarrow$ & (\%) $\downarrow$ & $\downarrow$ \\ 
\midrule
CTG no collision & 4.0  & 27.1   & 27.1                                                                          & -                                                                                          & \textbf{0.569}           \\
CTG off-road     & 11.4                                                                       & 34.1                                                                      & 45.5                                                                          & -                                                                                          & \textbf{0.569}           \\
CTG*~            & 21.84                                                                      &\textbf{ 0.13}                                                                      & 21.96                                                                         & 9.31                                                                                       & 0.754           \\
Ours             & \textbf{3.49}                                                                       & 0.87                                                                      & \textbf{4.18}                                                                          & \textbf{6.54}                                                                                       & 0.87                      \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Comparative Analysis in Closed-Loop Traffic Simulation.}  While our approach exhibits a slightly higher realism, it significantly outperforms both CTG versions in terms of reduced failure rate and improved wrong direction rate, highlighting the efficacy of our proposed guidance strategies.}

\label{tab:ctg}
\vspace{-1em}
\end{table}

==> tbl/ctrl_ctype.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{\textbf{Safety-critical Traffic Simulation.} We compare the our approach against STRIVE \cite{strive} for safety-critical traffic simulation with a rule-based planner. Our outperforms STRIVE on all metrics.}
\label{tab:strive2}
\begin{tabular}{l|ccccll} 
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Collision}   & \textbf{Adv Offroad} & \textbf{Realism}     & \textbf{Coll Angle var} & \textbf{Coll Rel Speed var}         & \textbf{\textbf{Coll point var}}   \\
                                 & (\%) $\uparrow$      & (\%) $\downarrow$    & $\downarrow$         & (deg) $\uparrow$        & (m/s) \$ \textbackslash{}uparrow \$ & (m) \$ \textbackslash{}uparrow \$  \\ 
\cmidrule{1-5}\cline{6-7}
baseline w/o \$J\_control\$      & 23.9                 & \textbf{13.8}        & 0.91                 & 2.22                    & \multicolumn{1}{c}{2.99}            & \multicolumn{1}{c}{1.62}           \\
+ Coll type control (PD)         & 29.0                 & 14.6                 & 0.57                 & 3.10                    & \multicolumn{1}{c}{1.96}            & \multicolumn{1}{c}{5.44}           \\
- \$J\_reg\$                     & 53.5                 & 23.1                 & 0.58                 & 3.34                    & \multicolumn{1}{c}{4.81}            & \multicolumn{1}{c}{2.47}           \\
                                 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    &                                     &                                    \\
\bottomrule
\end{tabular}
\end{table}


==> tbl/ddim_abl_sup.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc} 
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Coll Rate} & \textbf{Off Road} & \textbf{Failure Rate} & \textbf{Wrong Direction} & \textbf{Progress} & \textbf{Realism}  \\
                                 & (\%) $\downarrow$  & (\%) $\downarrow$  & (\%) $\downarrow$     & (\%) $\downarrow$        & (m) $\uparrow$    & $\downarrow$      \\ 
\midrule
DDIM (10 steps)                  & 3.58               & 5.34               & 8.78                  & 16.97                    & \textbf{65.4}     & 0.93              \\
DDIM (5 steps)                   & 3.79               & 9.53               & 12.84                 & 20.71                    & 62.4              & 0.83              \\
DDIM (1 step)                    & 3.47               & 11.16              & 14.03                 & 21.41                    & 58.9              & \textbf{0.53}     \\
DDPM (100 steps)                 & \textbf{1.74}      & \textbf{4.40}               & \textbf{6.05}         & \textbf{9.73}            & 51.3              & 0.88              \\
\bottomrule
\end{tabular}
}
\label{tab:ddim}
\caption{\textbf{Ablation Study on Accelerated Sampling through Different DDIM Steps.} The table illustrates a performance degradation with fewer diffusion steps. Notably, DDIM with 10 steps still maintains a relatively low failure rate.}

\end{table}


==> tbl/diff_planner_sup.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccccc} 
\toprule
\multicolumn{1}{c|}{\textbf{Planner}} & \textbf{Ego-Adv Coll} & \textbf{Ego-Other Coll} & \textbf{Adv Offroad} & \textbf{Coll Speed} & \textbf{Ego Accel } & \textbf{Realism}  \\
                                  & (\%) $\uparrow$       & (\%) $\uparrow$         & (\%) $\downarrow$    & (m/s) $\downarrow$  & (m/s\(^2\)) $\downarrow$             & $\downarrow$      \\ 
\midrule
BC                                & 40.3                  & 43.3                    & 20.9                 & 2.65                & 0.60                                   & 0.83              \\
IDM                               & \textbf{49.3}         & \textbf{58.2}           & 15.0                 & \textbf{-0.37}      & 1.09                                   & 0.85              \\
Lane-graph                        & 35.8                  & 38.8                    & \textbf{13.4}        & 2.34                & 2.51                                   & \textbf{0.60}     \\
\bottomrule
\end{tabular}
}
\captionof{table}{\textbf{Safety-Critical Simulation for different Planner settings}}
\label{tab:supp_diffplan}
\end{table}


==> tbl/strive.tex <==
\setlength\tabcolsep{4 pt}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc} 
\toprule
\multirow{2}{*}{\textbf{Method}}      & \multirow{2}{*}{\textbf{Collision}} & \textbf{Other}    & \textbf{Adv}      & \textbf{Collision} & \multirow{2}{*}{\textbf{Realism}}  \\
                                      &                                     & \textbf{Offroad}  & \textbf{Offroad}  & \textbf{Rel Speed} &                                    \\
                                      & (\%) $\uparrow$                     & (\%) $\downarrow$ & (\%) $\downarrow$ & (m/s) $\downarrow$ & $\downarrow$                       \\ 
\midrule
STRIVE                                & 36.4                                & 2.2               & \textbf{11.4}     & 5.52               & 0.85                               \\
Ours                                  & \textbf{43.2}                       & \textbf{1.9}      & \textbf{11.4}     & \textbf{-0.12}     & 0.38                               \\
\bottomrule
\end{tabular}
}
\vspace{.2em} 
\caption{\textbf{Safety-critical Traffic Simulation.} We compare our approach against STRIVE \cite{strive} for safety-critical traffic simulation with a rule-based planner. Our method outperforms STRIVE on all metrics. \vspace{-1em}}
\label{tab:strive}
\end{table}
\setlength\tabcolsep{6 pt}



